Robust Optimization for Non-Convex Objectives

We consider robust optimization problems, where the goal is to optimize in the worst case over a class of objective functions. We develop a reduction from robust improper optimization to Bayesian optimization: given an oracle that returns $\alpha$-approximate solutions for distributions over objectives, we compute a distribution over solutions that is $\alpha$-approximate in the worst case. We show that de-randomizing this solution is NP-hard in general, but can be done for a broad class of statistical learning tasks. We apply our results to robust neural network training and submodular optimization. We evaluate our approach experimentally on corrupted character classification, and robust influence maximization in networks.

==> applications.tex <==
\section{Applications}
\subsection{Neural Network Training}
%Intuitively, the reason why deep neural networks fail on inputs corrupted by adversarial noise is due to the fact that the noise is constructed so that points are pushed beyond decision boundaries.  To do so, the adversary needs to know the classification boundary created by the classifier and assume that it is \emph{fixed}.  If we have access to the noise generator and train a classifier on noisy images, the classifier will classify images well.  Thus, in this case, we can imagine that we have a set of noise types $N_{1},\ldots,N_{m}$ and for each $i \in [m]$ we are able to find a set of weights $\mathbf{x}_i \in \mathbb{R}^n$ s.t. the classification accuracy $f_i(\mathbf{x}_i)$ is at least some $\alpha$, where $\alpha \in [0,1]$\footnote{For example, for most noise distributions we tested, simple neural network architectures are able to produce solutions s.t. their accuracy $\alpha$ is over $90\%$.}.  If we know which noise type the adversary uses we can trivially train a classifier on that noise type and obtain accuracy of $\alpha$.  Since we do not know which noise type the adversary uses, our expected accuracy is at most $\alpha/k$, which goes to zero as $k$ grows. 

\paragraph{Classification via robust optimization with approximate oracles.}  In our setting, we can consider the weights we use to train a neural network as the space $\mathcal{X} \subseteq \mathbb{R}^n$ we aim to optimize over.  We have a set of noise types $N_{1},\ldots,N_{m}$ and for each $i \in [m]$ we can use $f_i:\mathcal{X} \to [0,1]$ to measure the accuracy of a weight vector $\mathbf{x} \in \mathcal{X}$.  Since there are no provable guarantees for training neural networks, we assume that we do not know how to optimize $f_i$ \emph{exactly}, but rather that there is some $\alpha\in [0,1]$ s.t. we know how to obtain a solution $\mathbf{x}_i \in \mathbb{R}^n$ s.t. $f(\mathbf{x}_i) \geq \alpha f_i(\mathbf{x}_i^\star)$, where $\mathbf{x}_i^\star$ is the weight vector that achieves optimal accuracy, i.e. $\mathbf{x}_i^\star \in \arg\max_{\mathbf{x}}f_i(\mathbf{x})$.  %In our context, each $f_i$ measures the \emph{accuracy} that a DNN can achieve when trained with noise generator $i \in [k]$.  Since we may not be able to train the DNN to have perfect or even optimal accuracy, we resort to this black-box model: if one assumes that the DNN can correctly classify at least $\alpha$ fraction of the inputs, our goal is to return a robust classifier whose accuracy is a function of $\alpha$.\footnote{Observe that by using this black-box approach we circumvent the issue that there are no guarantees for training DNNs.}    
Notice that the above implies that we have an $\alpha$ distributional oracle for the problem.  Let $p_{1},\ldots,p_{m}$ be a set of weights that sum to $1$, then:
%
$$\mathbb{E}[ f(M(D)) ] = \sum_{i=1}^{m}p_i f_i(\mathbf{x}_i) \geq \sum_{i=1}^{m}p_i \alpha f_i(\mathbf{x}^\star_i)  \geq \sum_{i=1}^{m}p_i \alpha f(\mathbf{x}^\star) = \alpha \max_{\mathbf{x} \in \mathcal{X}}\mathbb{E}_{f \sim \mathcal{F}}[f(\mathbf{x})]$$
%


\paragraph{Robust accuracy guarantees.}

Our goal is to find a solution $\mathbf{x}\in X$ that achieves good quality for all $f_i$. In particular, we seek the max-min optimal solution:
\begin{equation}
\mathbf{x}_{best} = \arg\max_{\mathbf{x}\in X}\min_{i\in [k]} f_i(\mathbf{x})
\end{equation}

\begin{corollary}
The algorithm returns a solution $\hat{\mathbf{x}}$ that for any noise type, obtains a bounded approximation (as a function of $\alpha$) to $\tau^\star = \min_{i\in [k]}f_{i}(\mathbf{x}_{best})$:
%
$$\min_{i \in [k]} f_i(\hat{\mathbf{x}}) \geq \alpha \tau^\star - o(1)$$
%
 \end{corollary}







Since we do not necessarily know the noise type that the adversary intends to use the question becomes: \emph{Given a set of weights $\mathbf{x}_1,\ldots,\mathbf{x}_k$ s.t. the accuracy of a DNN with $\mathbf{x}_i$ on noise type $N_i$ is at least $\alpha$, i.e. $\min_{i\in k} f(\mathbf{x}_i) \geq \alpha$, can we design a classifier whose accuracy approaches $\alpha$?}

\paragraph{Main steps in designing noise robust DNN architectures.} In this project our goal is to design a DNN that is robust to adversarial noise.  In particular, for any noise types, $N_1,\ldots,N_k$ for which one can achieve accuracy at least $\alpha$, our goal is to construct a DNN that can provably achieve accuracy $\alpha$ without knowing which noise type the adversary uses.  Our approach follows the following steps:

\begin{enumerate}
\item \textbf{Robust optimization with approximate oracles:} As a first step, we are interested in designing an algorithm that obtains max-min accuracy guarantees.  There are two major challenges: first, the accuracy functions are generally non-convex and optimization is highly non-trivial.  Second, we do not know how to optimize the accuracy functions exactly, but within some approximate accuracy $\alpha<1$;
\item \textbf{Training via boosting:} Our goal is to use boosting on the solutions $\mathbf{x}_1,\ldots,\mathbf{x}_k$ and obtain an algorithm with a max-min approximation guarantee;
\item \textbf{Classification from robust guarantees:} Next, given an algorithm for the max-min problem, we intend to use the algorithm to design a classifier whose accuracy approaches $\alpha$ by using various update methods used in online learning; 
\item \textbf{Implementation:} In order to implement the classifier we need to design a DNN architecture that trains using multiple classifiers.  We describe two complementary approaches that seem promising;
\item \textbf{Experimental setup:} Finally, we are interested in developing a testing methodology to evaluate the performance of our algorithms.  We describe several simple ways to generate noise types on the popular MNIST image data set.
\end{enumerate} 

Each step is discussed in detail in the sections below, together with performance metrics, major milestones  at intermediate stages of the project that can be used to demonstrate progress, followed by a comprehensive timeline. 


%We will consider the problem of image classification in neural networks, where images have been corrupted by an adversary and contain some noise that can misclassify an classifier as discussed above.    
%
%
%A key observation is that if we have access to the noise generator that was applied on the image, we can train a classifier using a noise generator in a matter that performs well.
%
%  
%but in the case where the image has been corrupted by noise.
%but in particular the case of having \textit{multiple} types of noise to \textsc{\char13}defend\textsc{\char13} against. We'll also assume slightly less sophisticated noise models than the adversarial noise from Goodfellow, Schlens, \& Szegedy. The primary challenge we'll address here is how to train the network to be robust against all these multiple types of noise simultaneously.
%
%Specifically, we focus on the following problem: given some image classification problem being approached using a neural network, suppose we also know the set of noises that could be present in the test data, and we have an algorithm to apply any of these noise types to our training data. We want to find a classifier (in this case, a set of weights for the neural network) that does as well as possible in test classification accuracy on all the noise types. That is, we want to prepare against the worst case by designing our classifier to do well in terms of the minimum of test accuracies across all noise types that could be present in the test data. We call this the problem of robust optimization.
%

\subsection*{1. Robust Optimization with Approximation Oracles}
First we discuss robust optimization at a general level, as a model of optimization under uncertainty.  At a high level, we will use this framework to model the uncertainty about the noise type the adversary applies, and our goal is to find a single solution (weights for the DNN) that is robust to the worst kind of noise the adversary can use.  



\subsection*{2. Training via boosting} 
In a boosting procedure, the idea is to iterate $T$ rounds, where in each iteration $t \in [T]$ we produce a distribution $D_t = (D_{t,1},...,D_{t,k})$ over the weights learned for each noise type $\mathbf{x}_1,...,\mathbf{x}_k$ (where we initialize $D_0$ as the discrete uniform distribution) and feed the distribution $D_t$ into an \emph{oracle}. The oracle selects some set of neural network weights $x_t$ (we will discuss different algorithms for this oracle later).  To train a classifier we will use an algorithm that yields solution set $x_1,...,x_T$.  Then we can compute the empirical accuracy $f$:
\begin{equation}
\mathbb{E}_{x_t \sim D_t} \left [ f(x_t) \right ] = \frac{1}{k}\sum_{i=1}^k D_{t,i} f_i(x_t)
\end{equation}


\paragraph{Designing the DNN architecture.}  In order to implement the boosting method, we need to evaluate different DNN architectures. In particular, we assume that the DNN has $\alpha$ accuracy, but this largely depends on its architecture and we need to evaluate its accuracy.  If we can compute $\mathbb{E}_{x\sim P}\left[f_i(x)\right]$ for each $i$ then for each noise type, we perturb the training data with it and compute the classification accuracy using each of the $T$ classifiers. We take the averages across all $T$ classifiers, and then finally find the smallest such average among noise types. This would give us an upper bound guarantee on how good the classification accuracy could possibly be for any classifier under this robust optimization framework, and gives us an idea of how good our set of classifiers is.

Design an algorithm to evaluate the accuracy $\alpha$ of a given DNN architecture.





\subsection{Robust Submodular Optimization}


\paragraph{Robust Submodular Maximization}
Consider the case where $\X\subseteq \{0,1\}^m$ is a subset of the power set over $m$ items and where each function $f\in\F$ is a submodular function. Since, the convex combination of submodular functions is also submodular, we get that when the feasible sets $\X$ forms a matroid, then there exits a polynomial time $(1-1/e)$-approximate distributional oracle. Therefore, Theorem \ref{thm:distributionally-robust-2}, yields the following corollary: 
\begin{corollary}
When $\X\subseteq \{0,1\}^m$ is a matroid set system and $\F$ contains only submodular functions, then there exists a polynomial time algorithm which computes a distribution $\Po$ over solutions, defined as a uniform distribution over a set $\{x_1,\ldots,x_T\}$, such that:
\begin{equation}
\min_{f\in \F} \E_{x\sim \Po}\left[f(x)\right] \geq \left( 1-\frac{1}{e} \right) \tau^*- \sqrt{\frac{2\log(|F|)}{T}}
\end{equation}
\end{corollary}

\paragraph{Alternative approach for robust coverage maximization}
When $\F$ contains functions only from the smaller set of coverage valuations and the feasibility set contains simple cardinality constraints, i.e. $\X= \{x\in \{0,1\}^m: |x| \leq k\}$, then we can achieve high probability robust guarantees rather than only in expectation guarantees. A coverage valuation is defined by a set of ground elements $E$. Each item $j\in [m]$ is then associated with a subset $C_j\subseteq E$ of ground elements that it covers. Each element $e$ is associated with a non-negative weight $w_e$. The value of the function for a set of items $x$ is the total weight of the elements that it covers: 
\[f(x) = \sum_{e\in E} w_e  {\bf 1}\{\exists j\in x: e\in C_j\}\]

Our approach here is very different from the previous section. We first note that coverage valuations admit a polynomially computable concave relaxation, i.e. for any coverage valuation $f:\{0,1\}^m\rightarrow R_+$, define the concave relaxation $F:[0,1]^m \rightarrow R_+$ as:
\begin{equation}
F(x) = \sum_{e\in E} w_e \min\left\{1,\sum_{j\in [m]: e\in C_j} x_j\right\}
\end{equation} 
By applying Corollary \ref{cor:convex} on the setting with solution space $\X' =\{ x\in [0,1]^m: \sum_i x_i \leq k\}$ and function space $\F' = \{F_1,\ldots, F_k\}$, where $F_i$ is the concave relaxation of function $f_i\in \F$, and the fact that convex programs are poly-time solvable we get:
\begin{corollary}\label{cor:concave-relax}
There exists an algorithm for computing a fractional solution $x^*\in [0,1]^m$, such that:
\begin{equation}
\min_{F\in \F} F(x^*) \geq \max_{x\in \X'}\min_{F\in \F'} F(x)- \sqrt{\frac{2\log(|F|)}{T}}
\end{equation}
The algorithm runs in time $\poly(|\F|,T)$ and makes $T$ calls to the distributional oracle.
\end{corollary}

Now observe that:
\begin{equation}
\max_{x\in X'}\min_{F\in \F'} F(x) \geq \max_{x\in \X} \min_{F\in \F'}F(x) = \max_{x\in \X} \min_{f\in \F}f(x)
\end{equation}

\begin{theorem}
Suppose that we have a randomized oblivious rounding scheme, that randomly maps any fractional solution $X$ into an integral solution $x$ independently of the function $f$, such that for each $f\in F$, with probability $1-\delta(\epsilon)$ it achieves:
\begin{equation}
f(x) \geq (1-\epsilon) F(X)
\end{equation}
and $\sum_i x_i \leq (1+\epsilon) k$.
Given access to any such oblivious rounding scheme we can compute an integral solution $x^*$ in polynomial time, that with probability at least $1-|\F|\delta$ it is:
\begin{itemize}
\item approximately feasible, i.e. $\sum_i x_i^*\leq (1+\epsilon) k$
\item it is $(1-\epsilon)$-approximately robust, i.e.:
\begin{equation}
\min_{f\in \F} f(x^*) \geq (1-\epsilon) \max_{x\in \X} \min_{f\in \F} f(x) - \sqrt{\frac{2\log(|F|)}{T}}
\end{equation}
\end{itemize} 
\end{theorem}
\begin{proof}
The theorem simply follows by applying the algorithm implied by Corollary \ref{cor:concave-relax} on the concave relaxations of the functions and then applying the oblivious rounding scheme for the relaxed solution returned by that algorithm. Then applying a union bound over all functions, gives us a guarantee on the minimum over function $f\in \F$.
\end{proof}

\subsection{Transfer Learning}



==> neural_network_experiment.tex <==
\section{Neural Network Experiments}

\subsection{Experiment Setup}

We use the MNIST handwritten digits data set containing $55000$ training images, $5000$ validation images, and $10000$ test images, each image being a $28 \times 28$ pixel grayscale image. The intensities of these $576$ pixels (ranging from $0$ to $1$) are used as input to a neural network that has $1024$ nodes in its one hidden layer. The output layer uses the softmax function to give a distribution over digits $0$ to $9$. The activation function is ReLU and the network is trained using Gradient Descent with learning parameter $0.5$ through $500$ iterations of mini-batches of size $100$. In the robust optimization procedure, we use the training set to fit classifiers, the validation set to perform multiplicative weight updates, and the test set to evaluate the performance of our classifiers.

\subsection{Oracle Baselines}

\begin{itemize}

\item \textbf{Individual Noise Baselines}: For each noise type $i$, we construct one such baseline oracle that trains a neural network using the training data perturbed by noise type $i$, and then returns the trained network weights as $x_t$, for every $t$. Notice that this oracle does not use $D_t$. This gives $k$ baselines, one for each noise type.

\item \textbf{Even Split Baseline}: We also consider another baseline which alternates between training with different noise types between iterations. In particular, call the previous $k$ baseline oracles as Oracle $1$,...,Oracle $k$. Then this new baseline oracle will produce $x_t$ just like Oracle $i + 1$, where $i \equiv t \mod k$.

\item \textbf{Uniform Distribution Baseline}: Finally, a more advanced baseline runs the robust optimization scheme with the Hybrid Method as described above, but without the distribution updates. Instead, the distribution over noise types is fixed as the discrete uniform $[\frac{1}{k},...,\frac{1}{k}]$ over the course of all $T$ iterations. This allows us to check if the multiplicative weight updates in the robust optimization algorithm are providing benefit.

\end{itemize}

\subsection{Noise Sets TODO}

\subsection{Neural Network Results TODO}

table

also, discuss number of trials, how need a scaled bound to ensure between 0 and 1,...

==> neural_network_theory.tex <==
\section{Neural Network Theory}

\subsection{Hybrid Method}

 \begin{center}
    \includegraphics[scale = .35,angle=0,origin=c]{figures/hybrid_method.png}
    \end{center}

For each iteration, given input $D_t = [D_{t,1},...,D_{t,k}]$, we take each training data image and perturb it by exactly one noise, with noise $i$ being selected with probability $D_{t,i}$ independently of the other images. Then apply mini-batch gradient descent, picking mini-batches from the perturbed data set, to train a classifier $x_t$. Note that the resulting classifier will take into account noise $i$ more when $D_{t,i}$ is larger.

\subsection{Composite Method} 

 \begin{center}
    \includegraphics[scale = .35,angle=0,origin=c]{figures/composite_method.png}
    \end{center}
    
This method is like the Hybrid Method in that it allocates how much weight to give each noise type based on $D_t$. In the Composite Method, at each iteration, we use $k$ copies of the training data, where copy $i$ has Noise Type $i$ applied to all training images. The new neural network architecture has $k$ sub-networks, each taking in one of the $k$ training data copies as input. They all share the same set of neural network weights, however.

During a step of neural network training, a mini-batch is selected from the original training image set, and the corresponding images in each of the $k$ training set copies are used to complete a step of forward-propogation for each of the $k$ sub-networks. This yields a loss function value $Loss_{t,i}$ for sub-network $i$. We then perform a single pass of backpropogation using the weighted average of the losses $\sum_{i=1}^k D_{t,i} Loss_{t,i}$ in order to update the weights (recall all $k$ sub-networks share the same set of weights). Perform this training method with many mini-batches, just like in standard neural network training, to obtain $x_t$.

\subsection{Loss Performance Criteria}

We consider two such criteria: \textbf{Individual Bottleneck Loss} and \textbf{Ensemble Bottleneck Loss}. Recall we are technically considering the negated loss, so that larger values correspond to better performance.

One way to judge the performance of sets of classifier solutions $P = Unif \{x_1,...,x_T\}$ is by maximizing the Individual Bottleneck Loss criterion $\min_{f \in F} E_{x \sim P} f(x)$, where $f$ is based on the test data. This criterion fits directly with the robust optimization theory bound in (XXX).

Note that simply running an algorithm that obtains $x_1,...,x_T$ for which $\min_{f \in F} E_{x \sim P} f(x)$ is large does not tell us how to make a prediction on new images. We can make predictions by using the following ensembling approach: For any given new image, for each classifier $x_t$, obtain the $10$ softmax output layer values $v_{t,0},..,v_{t,9}$, one for each digit. Then the prediction is $\argmax_{d \in \{0,...,9\}} \sum_t v_{t,d}$.

Meanwhile, the cross entropy between $[\frac{1}{T} \sum_{t=1}^T v_{t,0},...,\frac{1}{T} \sum_{t=1}^T v_{t,9}]$ and the true one-hot-encoded label for an image is the ensemble-based loss associated with a given image. The mean over many images is the ensemble-based loss over that set of images. Define the Ensemble Bottleneck Loss for a set of images as the worst mean loss for that set of images perturbed by each noise type $i=1,...,k$. This criterion fits directly with the robust optimization theory bound in (XXX).
